Inside the Muchnik Degrees I: Discontinuity, Learnability, and Constructivism

Every computable function has to be continuous. To develop computability theory of discontinuous functions, we study low levels of the arithmetical hierarchy of nonuniformly computable functions on Baire space. First, we classify nonuniformly computable functions on Baire space from the viewpoint of learning theory and piecewise computability. For instance, we show that mind-change-bounded-learnability is equivalent to finite $(\Pi^0_1)_2$-piecewise computability (where $(\Pi^0_1)_2$ denotes the difference of two $\Pi^0_1$ sets), error-bounded-learnability is equivalent to finite $\Delta^0_2$-piecewise computability, and learnability is equivalent to countable $\Pi^0_1$-piecewise computability (equivalently, countable $\Sigma^0_2$-piecewise computability). Second, we introduce disjunction-like operations such as the coproduct based on BHK-like interpretations, and then, we see that these operations induce Galois connections between the Medvedev degree structure and associated Medvedev/Muchnik-like degree structures. Finally, we interpret these results in the context of the Weihrauch degrees and Wadge-like games.

==> figure/cross.tex <==
\[
	\begin{xy}
%	(0,84) *{\cross^1_1}="1-1",
	(30,90) *{(Medvedev\ complete)},
%
	(0,72) *{\cross^1_2\ \ }="1-2",
	(15,76) *{\ \ \cross^2_3\ \ }="2-3",
	(30,80) *{\ \ \cross^3_4\ \ }="3-4",
	(45,84) *{\ \ \cross^4_5\ \ }="4-5",
	(60,88) *{\ \ \cross^5_6\ \ }="5-6",
	(75,92) *{\ \ \cross^6_7\ \ }="6-7",
	(90,96) *{\ \ \cross^7_8\ \ }="7-8",
	(105,100) ="8-9",
%
	(0,60) *{\cross^1_3\ \ }="1-3",
	(15,64) *{\ \ \cross^2_4\ \ }="2-4",
	(30,68) *{\ \ \cross^3_5\ \ }="3-5",
	(45,72) *{\ \ \cross^4_6\ \ }="4-6",
	(60,76) *{\ \ \cross^5_7\ \ }="5-7",
	(75,80) *{\ \ \cross^6_8\ \ }="6-8",
	(90,84) *{\ \ \cross^7_9\ \ }="7-9",
	(105,88) ="8-10",
%
	(0,48) *{\cross^1_4\ \ }="1-4",
	(15,52) *{\ \ \cross^2_5\ \ }="2-5",
	(30,56) *{\ \ \cross^3_6\ \ }="3-6",
	(45,60) *{\ \ \cross^4_7\ \ }="4-7",
	(60,64) *{\ \ \cross^5_8\ \ }="5-8",
	(75,68) *{\ \ \cross^6_9\ \ }="6-9",
	(90,72) *{\ \ \cross^7_{10}\ \ }="7-10",
	(105,76) ="8-11",
%
	(0,36) *{\cross^1_5\ \ }="1-5",
	(15,40) *{\ \ \cross^2_6\ \ }="2-6",
	(30,44) *{\ \ \cross^3_7\ \ }="3-7",
	(45,48) *{\ \ \cross^4_8\ \ }="4-8",
	(60,52) *{\ \ \cross^5_9\ \ }="5-9",
	(75,56) *{\ \ \cross^6_{10}\ \ }="6-10",
	(90,60) *{\ \ \cross^7_{11}\ \ }="7-11",
	(105,64) ="8-12",
%
	(0,24) *{\cross^1_6\ \ }="1-6",
	(15,28) *{\ \ \cross^2_7\ \ }="2-7",
	(30,32) *{\ \ \cross^3_8\ \ }="3-8",
	(45,36) *{\ \ \cross^4_9\ \ }="4-9",
	(60,40) *{\ \ \cross^5_{10}\ \ }="5-10",
	(75,44) *{\ \ \cross^6_{11}\ \ }="6-11",
	(90,48) *{\ \ \cross^7_{12}\ \ }="7-12",
	(105,52) ="8-13",
%
	(0,12) *{\ \ }="1-7",
	(15,16) *{\ \ \ \ }="2-8",
	(30,20) *{\ \ \ \ }="3-9",
	(45,24) *{\ \ \ \ }="4-10",
	(60,28) *{\ \ \ \ }="5-11",
	(75,32) *{\ \ \ \ }="6-12",
	(90,36) *{\ \ \ \ }="7-13",
	(105,40) ="8-14",
%
	(-14,70) *{(connected)},
	(-18,58) *{(simply\ connected)},
	(-14,46) *{(2\mbox{-}connected)},
	(-14,34) *{(3\mbox{-}connected)},
	(-14,22) *{(4\mbox{-}connected)},
%
	\ar @{.} (-15,62);(105,94)
	\ar @{.} (-15,50);(105,82)
	\ar @{.} (-15,38);(105,70)
	\ar @{.} (-15,26);(105,58)
	\ar @{.} (-15,14);(105,46)
%
	\ar @{.} (-9,84);(81,36)
%
	\ar "2-3";"1-2"
	\ar "3-4";"2-3"
	\ar "4-5";"3-4"
	\ar "5-6";"4-5"
	\ar "6-7";"5-6"
	\ar "7-8";"6-7"
	\ar "8-9";"7-8"
%
	\ar "2-4";"1-3"
	\ar "3-5";"2-4"
	\ar "4-6";"3-5"
	\ar "5-7";"4-6"
	\ar "6-8";"5-7"
	\ar "7-9";"6-8"
	\ar "8-10";"7-9"
%
	\ar "2-5";"1-4"
	\ar "3-6";"2-5"
	\ar "4-7";"3-6"
	\ar "5-8";"4-7"
	\ar "6-9";"5-8"
	\ar "7-10";"6-9"
	\ar "8-11";"7-10"
%
	\ar "2-6";"1-5"
	\ar "3-7";"2-6"
	\ar "4-8";"3-7"
	\ar "5-9";"4-8"
	\ar "6-10";"5-9"
	\ar "7-11";"6-10"
	\ar "8-12";"7-11"
%
	\ar "2-7";"1-6"
	\ar "3-8";"2-7"
	\ar "4-9";"3-8"
	\ar "5-10";"4-9"
	\ar "6-11";"5-10"
	\ar "7-12";"6-11"
	\ar "8-13";"7-12"
%
	\ar "1-2"+/d.3cm/ ;"1-3"+/u.3cm/
	\ar "2-3"+/d.3cm/ ;"2-4"+/u.3cm/
	\ar "3-4"+/d.3cm/ ;"3-5"+/u.3cm/
	\ar "4-5"+/d.3cm/ ;"4-6"+/u.3cm/
	\ar "5-6"+/d.3cm/ ;"5-7"+/u.3cm/
	\ar "6-7"+/d.3cm/ ;"6-8"+/u.3cm/
	\ar "7-8"+/d.3cm/ ;"7-9"+/u.3cm/
%
	\ar "1-3"+/d.3cm/ ;"1-4"+/u.3cm/
	\ar "2-4"+/d.3cm/ ;"2-5"+/u.3cm/
	\ar "3-5"+/d.3cm/ ;"3-6"+/u.3cm/
	\ar "4-6"+/d.3cm/ ;"4-7"+/u.3cm/
	\ar "5-7"+/d.3cm/ ;"5-8"+/u.3cm/
	\ar "6-8"+/d.3cm/ ;"6-9"+/u.3cm/
	\ar "7-9"+/d.3cm/ ;"7-10"+/u.3cm/
%
	\ar "1-4"+/d.3cm/ ;"1-5"+/u.3cm/
	\ar "2-5"+/d.3cm/ ;"2-6"+/u.3cm/
	\ar "3-6"+/d.3cm/ ;"3-7"+/u.3cm/
	\ar "4-7"+/d.3cm/ ;"4-8"+/u.3cm/
	\ar "5-8"+/d.3cm/ ;"5-9"+/u.3cm/
	\ar "6-9"+/d.3cm/ ;"6-10"+/u.3cm/
	\ar "7-10"+/d.3cm/ ;"7-11"+/u.3cm/
%
	\ar "1-5"+/d.3cm/ ;"1-6"+/u.3cm/
	\ar "2-6"+/d.3cm/ ;"2-7"+/u.3cm/
	\ar "3-7"+/d.3cm/ ;"3-8"+/u.3cm/
	\ar "4-8"+/d.3cm/ ;"4-9"+/u.3cm/
	\ar "5-9"+/d.3cm/ ;"5-10"+/u.3cm/
	\ar "6-10"+/d.3cm/ ;"6-11"+/u.3cm/
	\ar "7-11"+/d.3cm/ ;"7-12"+/u.3cm/
%
	\ar "1-6"+/d.3cm/ ;"1-7"+/u.3cm/
	\ar "2-7"+/d.3cm/ ;"2-8"+/u.3cm/
	\ar "3-8"+/d.3cm/ ;"3-9"+/u.3cm/
	\ar "4-9"+/d.3cm/ ;"4-10"+/u.3cm/
	\ar "5-10"+/d.3cm/ ;"5-11"+/u.3cm/
	\ar "6-11"+/d.3cm/ ;"6-12"+/u.3cm/
	\ar "7-12"+/d.3cm/ ;"7-13"+/u.3cm/
	\end{xy}
\]

==> figure/cross_2.tex <==

\[
	\begin{xy}
	(15,88) *{\ \ \cross^n_m\ \ }="2-3",
%
	(0,60) *{\ \ }="1-3",
	(45,72) *{\ \ \cross^{kn}_{km}\ \ }="4-6",
%
	(45,48) *{\!\!\cross^{kn}_{(k+1)m-n-1}\!\!\!\!\!\!\!\!\!\!}="4-8",
	(60,52) *{\cross^{kn+1}_{(k+1)m-n}\!\!\!\!\!\!}="5-9",
%
	(45,36) *{\!\!\cross^{kn}_{(k+1)m-n}\!\!\!\!\!\!}="4-9",
	(60,40) *{\cross^{kn+1}_{(k+1)m-n+1}\!\!\!\!\!\!\!\!\!\!}="5-10",
	(90,48) *{\cross^{(k+1)n}_{(k+1)m}\!\!}="7-12",
	(105,52) ="8-13",
%
	(90,36) *{\ \ \ \ }="7-13",
%
	\ar @{.} (0,66);(52.5,80)
	\ar @{.} (52.5,80);(52.5,44)
	\ar @{.} (52.5,44);(97.5,56)
	\ar @{.} (97.5,56);(97.5,38)
%
	\ar "4-6";"1-3"
	\ar "5-9";"4-8"
	\ar "5-10";"4-9"
	\ar "7-12";"5-10"
%
	\ar "4-6"+/d.3cm/ ;"4-8"+/u.3cm/
	\ar "4-8"+/d.3cm/ ;"4-9"+/u.3cm/
	\ar "5-9"+/d.3cm/ ;"5-10"+/u.3cm/
	\ar "7-12"+/d.3cm/ ;"7-13"+/u.3cm/
%
	\ar @<1mm> "2-3";"4-6"
	\ar @{-->} @<1mm> @/^2.5pc/ "2-3";"5-9"|{\varprod}
	\ar @<1mm> @(u,u) @/^4pc/ "2-3";"7-12"
	\end{xy}
\]

==> figure/cross_ss.tex <==
\[
	\begin{xy}
%
	(0,72) *{\cross^1_2\ \ }="1-2",
	(15,76) *{\ \ \cross^2_3\ \ }="2-3",
	(30,80) *{\ \ \cross^3_4\ \ }="3-4",
	(45,84) *{\ \ \cross^4_5\ \ }="4-5",
	(60,88) *{\ \ \cross^5_6\ \ }="5-6",
	(75,92) *{\ \ \cross^6_7\ \ }="6-7",
	(90,96) *{\ \ \cross^7_8\ \ }="7-8",
	(105,100) ="8-9",
%
	(0,60) *{\cross^1_3\ \ }="1-3",
	(15,64) *{\ \ \cross^2_4\ \ }="2-4",
	(30,68) *{\ \ \cross^3_5\ \ }="3-5",
	(45,72) *{\ \ \cross^4_6\ \ }="4-6",
	(60,76) *{\ \ \cross^5_7\ \ }="5-7",
	(75,80) *{\ \ \cross^6_8\ \ }="6-8",
	(90,84) *{\ \ \cross^7_9\ \ }="7-9",
	(105,88) ="8-10",
%
	(0,48) *{\cross^1_4\ \ }="1-4",
	(15,52) *{\ \ \cross^2_5\ \ }="2-5",
	(30,56) *{\ \ \cross^3_6\ \ }="3-6",
	(45,60) *{\ \ \cross^4_7\ \ }="4-7",
	(60,64) *{\ \ \cross^5_8\ \ }="5-8",
	(75,68) *{\ \ \cross^6_9\ \ }="6-9",
	(90,72) *{\ \ \cross^7_{10}\ \ }="7-10",
	(105,76) ="8-11",
%
	(0,36) *{\cross^1_5\ \ }="1-5",
	(15,40) *{\ \ \cross^2_6\ \ }="2-6",
	(30,44) *{\ \ \cross^3_7\ \ }="3-7",
	(45,48) *{\ \ \cross^4_8\ \ }="4-8",
	(60,52) *{\ \ \cross^5_9\ \ }="5-9",
	(75,56) *{\ \ \cross^6_{10}\ \ }="6-10",
	(90,60) *{\ \ \cross^7_{11}\ \ }="7-11",
	(105,64) ="8-12",
%
	(0,24) *{\cross^1_6\ \ }="1-6",
	(15,28) *{\ \ \cross^2_7\ \ }="2-7",
	(30,32) *{\ \ \cross^3_8\ \ }="3-8",
	(45,36) *{\ \ \cross^4_9\ \ }="4-9",
	(60,40) *{\ \ \cross^5_{10}\ \ }="5-10",
	(75,44) *{\ \ \cross^6_{11}\ \ }="6-11",
	(90,48) *{\ \ \cross^7_{12}\ \ }="7-12",
	(105,52) ="8-13",
%
	(0,12) *{\ \ }="1-7",
	(15,16) *{\ \ \ \ }="2-8",
	(30,20) *{\ \ \ \ }="3-9",
	(45,24) *{\ \ \ \ }="4-10",
	(60,28) *{\ \ \ \ }="5-11",
	(75,32) *{\ \ \ \ }="6-12",
	(90,36) *{\ \ \ \ }="7-13",
	(105,40) ="8-14",
%
	(-14,70) *{(connected)},
	(-18,58) *{(simply\ connected)},
	(-14,46) *{(2\mbox{-}connected)},
	(-14,34) *{(3\mbox{-}connected)},
	(-14,22) *{(4\mbox{-}connected)},
%
	\ar @{.} (-15,62);(105,94)
	\ar @{.} (-15,50);(105,82)
	\ar @{.} (-15,38);(105,70)
	\ar @{.} (-15,26);(105,58)
	\ar @{.} (-15,14);(105,46)
%
%
	\ar "2-3";"1-2"
	\ar "3-4";"2-3"
	\ar "4-5";"3-4"
	\ar "5-6";"4-5"
	\ar "6-7";"5-6"
	\ar "7-8";"6-7"
	\ar "8-9";"7-8"
%
	\ar "2-4";"1-3"
	\ar "3-5";"2-4"
	\ar "4-6";"3-5"
	\ar "5-7";"4-6"
	\ar "6-8";"5-7"
	\ar "7-9";"6-8"
	\ar "8-10";"7-9"
%
	\ar "2-5";"1-4"
	\ar "3-6";"2-5"
	\ar "4-7";"3-6"
	\ar "5-8";"4-7"
	\ar "6-9";"5-8"
	\ar "7-10";"6-9"
	\ar "8-11";"7-10"
%
	\ar "2-6";"1-5"
	\ar "3-7";"2-6"
	\ar "4-8";"3-7"
	\ar "5-9";"4-8"
	\ar "6-10";"5-9"
	\ar "7-11";"6-10"
	\ar "8-12";"7-11"
%
	\ar "2-7";"1-6"
	\ar "3-8";"2-7"
	\ar "4-9";"3-8"
	\ar "5-10";"4-9"
	\ar "6-11";"5-10"
	\ar "7-12";"6-11"
	\ar "8-13";"7-12"
%
	\ar "1-2"+/d.3cm/ ;"1-3"+/u.3cm/
	\ar "2-3"+/d.3cm/ ;"2-4"+/u.3cm/
	\ar "3-4"+/d.3cm/ ;"3-5"+/u.3cm/
	\ar "4-5"+/d.3cm/ ;"4-6"+/u.3cm/
	\ar "5-6"+/d.3cm/ ;"5-7"+/u.3cm/
	\ar "6-7"+/d.3cm/ ;"6-8"+/u.3cm/
	\ar "7-8"+/d.3cm/ ;"7-9"+/u.3cm/
%
	\ar "1-3"+/d.3cm/ ;"1-4"+/u.3cm/
	\ar "2-4"+/d.3cm/ ;"2-5"+/u.3cm/
	\ar "3-5"+/d.3cm/ ;"3-6"+/u.3cm/
	\ar "4-6"+/d.3cm/ ;"4-7"+/u.3cm/
	\ar "5-7"+/d.3cm/ ;"5-8"+/u.3cm/
	\ar "6-8"+/d.3cm/ ;"6-9"+/u.3cm/
	\ar "7-9"+/d.3cm/ ;"7-10"+/u.3cm/
%
	\ar "1-4"+/d.3cm/ ;"1-5"+/u.3cm/
	\ar "2-5"+/d.3cm/ ;"2-6"+/u.3cm/
	\ar "3-6"+/d.3cm/ ;"3-7"+/u.3cm/
	\ar "4-7"+/d.3cm/ ;"4-8"+/u.3cm/
	\ar "5-8"+/d.3cm/ ;"5-9"+/u.3cm/
	\ar "6-9"+/d.3cm/ ;"6-10"+/u.3cm/
	\ar "7-10"+/d.3cm/ ;"7-11"+/u.3cm/
%
	\ar "1-5"+/d.3cm/ ;"1-6"+/u.3cm/
	\ar "2-6"+/d.3cm/ ;"2-7"+/u.3cm/
	\ar "3-7"+/d.3cm/ ;"3-8"+/u.3cm/
	\ar "4-8"+/d.3cm/ ;"4-9"+/u.3cm/
	\ar "5-9"+/d.3cm/ ;"5-10"+/u.3cm/
	\ar "6-10"+/d.3cm/ ;"6-11"+/u.3cm/
	\ar "7-11"+/d.3cm/ ;"7-12"+/u.3cm/
%
	\ar "1-6"+/d.3cm/ ;"1-7"+/u.3cm/
	\ar "2-7"+/d.3cm/ ;"2-8"+/u.3cm/
	\ar "3-8"+/d.3cm/ ;"3-9"+/u.3cm/
	\ar "4-9"+/d.3cm/ ;"4-10"+/u.3cm/
	\ar "5-10"+/d.3cm/ ;"5-11"+/u.3cm/
	\ar "6-11"+/d.3cm/ ;"6-12"+/u.3cm/
	\ar "7-12"+/d.3cm/ ;"7-13"+/u.3cm/
	\end{xy}
\]
